Controllability and Tracking of Ensembles: An Optimal Transport Theory Viewpoint

This paper explores the controllability and state tracking of ensembles from the perspective of optimal transport theory. Ensembles, characterized as collections of systems evolving under the same dynamics but with varying initial conditions, are a fundamental concept in control theory and applications. By leveraging optimal transport, we provide a novel framework for analyzing and solving the state tracking problem of ensembles, particularly when state observations are limited and only accessible at discrete time points. This study establishes connections between the ensemble dynamics and finite-horizon optimal control problems, demonstrating that the problem can be reformulated as a computationally efficient linear program using Kantorovich's formulation of optimal transport. We raise notions of observability and controllability for nonlinear ensembles, and propose methods for state tracking in Gaussian output distributions settings. Numerical examples and theoretical insights are provided to validate the approach, highlighting the utility of optimal transport in ensemble control problems.

==> Abstract.tex <==
%Abstract Page

\hbox{\ }

\renewcommand{\baselinestretch}{1}
\small \normalsize

\begin{center}
\large{{ABSTRACT}}

\vspace{3em}

\end{center}
\hspace{-.15in}
\begin{tabular}{ll}
Title of Dissertation:    & {\large  CONTROLLABILITY AND TRACKING OF ENSEMBLES:}\\
&                     {\large  AN OPTIMAL TRANSPORT THEORY VIEWPOINT} \\
\ \\
&                          {\large  Reza Hadadi} \\
&                           {\large Master of Science, 2021} \\
\ \\
Thesis Directed by: & {\large  Professor Eyad H. Abed} \\
&               {\large  Department of Electrical and Computer Engineering } \\
\end{tabular}

\vspace{3em}

\renewcommand{\baselinestretch}{2}
\large \normalsize


Ensembles are considered that are collections of systems (elements, agents, particles, or the like) in which the evolution of each component system is governed by the same dynamical equation, but with different initial conditions. In the context of controlling ensembles, it is assumed that the control inputs are uniformly applied to all of the systems within an ensemble (usually referred to as broadcast control). It is also assumed that the systems are not individually distinguishable. Instead, collections of their outputs are observed at certain time instants, without identifying indices or labels. 

In this regard, the notion of ensemble observability is reviewed and its relationship with the classical notion of observability for dynamical systems is studied first. Second, by characterizing the deterministic state distributions of ensembles as probability distributions over the state space, the state tracking problem for ensembles with linear dynamics which are optimally controlled with respect to some cost function is cast as an optimization problem over probability distributions. Third, an optimal transport (OT) theory viewpoint is adopted to transform the optimization problem into a linear programming problem to which numerical algorithms are applied, and the time-varying state distribution of the ensemble states is obtained.

Finally, the notion of ensemble controllability together with a proposed continuous measure of controllablity for nonlinear ensembles is proposed.

==> Acknowledgements.tex <==
%Acknowledgments

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{.5in}

\begin{center}
\large{Acknowledgements} 
\end{center} 

\vspace{1ex}
To be added ...
%First, I would like to thank the benevolent God whose presence in my mind has always been a source of calmness and resilience in the hard times.

%Among the people whom I am indebted the most in writing this thesis I should first mention my advisor Dr. Eyad Abed who trusted in my abilities in doing the current research and helped me out in any ways possible. He always provided great comments during the meetings and I do not forget his kind attitude even at the times of pointing out my mistakes.

%Last but not the least, I would like to take this opportunity to express my utmost gratitude towards my family, especially my dear wife, Shadi, whose constant support and tolerance made completing this thesis possible.

==> Copyright.tex <==
%Copyright

\thispagestyle{empty}
\hbox{\ }

\vfill
\renewcommand{\baselinestretch}{1}
\small\normalsize

\vspace{.5in}

\begin{center}
\large{\copyright \hbox{ }Copyright by\\
Reza Hadadi  %Type your name as it appears in University records
\\
2021}
\end{center}

\vfill

\newpage 


==> Dedication.tex <==
%Dedication

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{.5in}

\begin{center}
\large{Dedication}
\end{center} 

If needed.


==> Foreword.tex <==
%Foreword

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{.5in}

\begin{center}
\large{Foreword} 
\end{center} 

If needed.


==> Preface.tex <==
%Preface
\pagestyle{plain}\pagenumbering{roman} \setcounter{page}{2}
\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }

\vspace{.5in}

\begin{center}
\large{Preface}
\end{center}


If needed.


==> Titlepage.tex <==
%Titlepage

\thispagestyle{empty}
\hbox{\ }
\vspace{1in}
\renewcommand{\baselinestretch}{1}
\small\normalsize
\begin{center}

\large{{CONTROLLABILITY AND TRACKING OF ENSEMBLES: \\
AN OPTIMAL TRANSPORT THEORY VIEWPOINT}}\\
(Draft: Nov. 26, 2021)
\ \\
\ \\
\large{by} \\
\ \\
\large{Reza Hadadi}%Your full name as it appears in University records.
\ \\
\ \\
\ \\
\ \\
\normalsize
Thesis submitted to the Faculty of the Graduate School of the \\
University of Maryland, College Park in partial fulfillment \\
of the requirements for the degree of \\
Master of Science \\
2021
\end{center}

\vspace{7.5em}

\noindent Advisory Committee: \\
Professor Eyad H. Abed, Chair/Advisor \\
Professor Andr\'{e} Tits \\
Professor Radu V. Balan \\
Professor Derek Paley 

==> Titlepage2.tex <==
%Titlepage

\thispagestyle{empty}
\hbox{\ }
\vspace{1in}
\renewcommand{\baselinestretch}{1}
\small\normalsize
\begin{center}

M.S. Scholarly Paper\\
\large{{CONTROLLABILITY AND TRACKING OF ENSEMBLES: \\
AN OPTIMAL TRANSPORT THEORY VIEWPOINT}}\\

\ \\
\ \\
\large{Author: Reza Hadadi}\\
Advisor: Professor Eyad H. Abed\\
Second Reader: Professor Andre Tits%Your full name as it appears in University records.
\normalsize
\ \\ 
\ \\
Department of Electrical and Computer Engineering\\
University of Maryland, College Park\\
December 2021
\end{center}

\vspace{7.5em}


